Super-Resolution Appearance Transfer for 4D Human Performances

A common problem in the 4D reconstruction of people from multi-view video is the quality of the captured dynamic texture appearance which depends on both the camera resolution and capture volume. Typically the requirement to frame cameras to capture the volume of a dynamic performance ($>50m^3$) results in the person occupying only a small proportion $<$ 10% of the field of view. Even with ultra high-definition 4k video acquisition this results in sampling the person at less-than standard definition 0.5k video resolution resulting in low-quality rendering. In this paper we propose a solution to this problem through super-resolution appearance transfer from a static high-resolution appearance capture rig using digital stills cameras ($> 8k$) to capture the person in a small volume ($<8m^3$). A pipeline is proposed for super-resolution appearance transfer from high-resolution static capture to dynamic video performance capture to produce super-resolution dynamic textures. This addresses two key problems: colour mapping between different camera systems; and dynamic texture map super-resolution using a learnt model. Comparative evaluation demonstrates a significant qualitative and quantitative improvement in rendering the 4D performance capture with super-resolution dynamic texture appearance. The proposed approach reproduces the high-resolution detail of the static capture whilst maintaining the appearance dynamics of the captured video.

==> srat/image_files/4drec.tex <==
\begin{huge}


\begin{tabular}{ccc}
             \includegraphics[width=0.8\linewidth]{img/relight.png} & \includegraphics[width=1.1\linewidth]{img/livecap.png} &
             \includegraphics[width=1.4\linewidth]{img/mulay.png} \\
             \huge{(a)} & \huge{(b)} &
             \huge{(c)}  \\
            
        \end{tabular}
\end{huge}

==> srat/image_files/colour_correx.tex <==
\begin{subfigure}{.23\textwidth}
  \centering
  % include third image
  \includegraphics[width=1.\linewidth]{img/06_HR.png}  
  \subcaption{Original frame.}
  \label{fig:sub-third}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include fourth image
  \includegraphics[width=1.\linewidth]{img/06_corr.png}  
  \subcaption{Corrected frame.}
  \label{fig:sub-fourth}
\end{subfigure}

==> srat/image_files/couple_id.tex <==




% \begin{tabular}{M{30mm}M{30mm}}
\begin{huge}


\begin{tabular}{cc}
             \includegraphics[width=1.1\linewidth]{img/0203tex.png} & \includegraphics[width=1.1\linewidth]{img/0168tex.png} \\
             \huge{(a) $T_p(I_{LR})$} & \huge{(b) $T_p(I_{HR})$}\\
            \includegraphics[width=1.1\linewidth]{img/0203.png}  &
             \includegraphics[width=1.1\linewidth]{img/0168.png}  \\ 
             \huge{(c) $I_{LR}$} &\huge{(d) $I_{HR}$} \\
            
        \end{tabular}
\end{huge}

%   \begin{subfigure}{.50\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1.\linewidth]{img/0203tex.png}  
%   \caption{$T_p(I_f)$}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{.50\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=1.0\linewidth]{img/0168tex.png}  
%   \caption{$T_p(I_{HR})$}
%   \label{fig:sub-second}
% \end{subfigure}

% \begin{subfigure}{.50\textwidth}
%   \centering
  
%   \includegraphics[width=1.\linewidth]{img/0203.png}  
%   \caption{$I_f$}
%   \label{fig:sub-third}
% \end{subfigure}
% \begin{subfigure}{.50\textwidth}
%   \centering
%   % include fourth image
%   \includegraphics[width=1.\linewidth]{img/0168.png}  
%   \caption{$I_{HR}$}
%   \label{fig:sub-fourth}
% \end{subfigure}

==> srat/image_files/interaciton.tex <==
\begin{subfigure}{.23\textwidth}
  \centering
  % include third image
  \includegraphics[width=1.\linewidth]{img/interaction/interac_orig.png}  
  \caption{Original.}
  \label{fig:sub-third}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include fourth image
  \includegraphics[width=1.\linewidth]{img/interaction/interac_corr.png}  
  \caption{SRAT output.}
  \label{fig:sub-fourth}
\end{subfigure}

==> srat/image_files/modelout.tex <==
\begin{tiny}


% \begin{tabular}{M{100mm}}
\begin{tabular}{c}
LR\\
\includegraphics[width=0.475\linewidth]{img/juliet/orig.png} \\  
2x SR\\
\includegraphics[width=0.475\linewidth]{img/juliet/x2.png}  \\
4x SR\\
\includegraphics[width=0.475\linewidth]{img/juliet/detailsx4.png}  \\
\end{tabular}
\end{tiny}

==> srat/image_files/modelout2_new.tex <==
\begin{huge}
\begin{tabular}{cc}
Output model & Original LR\\
\includegraphics[width=1\linewidth]{img/juliet/final_modelj.png} &
\includegraphics[width=1\linewidth]{img/new/jul3.png} \\  
Corrected LR & 2x SR\\
\includegraphics[width=1\linewidth]{img/new/jul2.png}  &
\includegraphics[width=1\linewidth]{img/new/jul1.png}  \\
\end{tabular}
\end{huge}

==> srat/image_files/network.tex <==
\includegraphics[width=1.\linewidth]{img/network.png} 

==> srat/image_files/patches.tex <==
\begin{tabular}{cccc}
                      
             
             \includegraphics[width=1in]{img/img5.jpg} & \includegraphics[width=1in]{img/img7.jpg} & \includegraphics[width=1in]{img/05469.png} & \includegraphics[width=1in]{img/06290.png} 
        \end{tabular}

==> srat/image_files/stasr.tex <==



\begin{tabular}{c}
             \includegraphics[width=1.1\linewidth]{img/SR1.png} \\
             (a) \cite{li20193d} \\
             \includegraphics[width=1.1\linewidth]{img/SR2.png}\\
             (b) \cite{richard2019learned}\\
        \end{tabular}


==> srat/image_files/supcc1_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{cccc}
 &  & \multicolumn{2}{c}{\multirow{2}{*}{\includegraphics[width=1.4in]{img/juliet/02202.png}}} \\
 &  & \multicolumn{2}{c}{}                 
\end{tabular}

==> srat/table/SR1_conf.tex <==
\begin{tabular}{|c|c|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Models}} & \multicolumn{1}{c|}{\multirow{2}{*}{Scale}} & \multicolumn{2}{c|}{SingleF}                          & \multicolumn{2}{c|}{SingleM}                          \\ \cline{3-6} 
\multicolumn{1}{|c|}{}                                & \multicolumn{1}{|c}{}                       & \multicolumn{1}{|c}{PSNR\uparrow} & \multicolumn{1}{|c}{SSIM\uparrow} & \multicolumn{1}{|c}{PSNR\uparrow} & \multicolumn{1}{|c|}{SSIM\uparrow} \\ \hline
1a                                                    & 2x                                          & 48.53                     & 0.9910                    & 50.31                     & 0.9935                    \\
1b                                                    & 2x                                          & {\textbf{48.64}}      & {\textbf{0.9912}}     & {\textbf{50.45}}      & { \textbf{0.9937}}     \\
1c                                                    & 2x                                          & 48.60                     & 0.9910                    & 50.41                     & 0.9937                    \\
2a                                                    & 2x                                          & 47.68                     & 0.9892                    &    48.91                       &      0.9914                     \\
2b                                                    & 2x                                          & 47.70                     & 0.9893                    &     48.94                      &        0.9915                   \\
2c                                                    & 2x                                          & 47.77                     & 0.9895                    &      40.01                     &             0.9916              \\
3a                                                    & 2x                                          & 47.74                     & 0.9893                    &        48.92                   &           0.9915                \\
3b                                                    & 2x                                          & 47.85                    & 0.9895                    &       49.22                    &         0.9918                  \\
3c                                                    & 2x                                          & 28.68                     & 0.8737                    &         49.33                  &          0.0019                 \\
                                                                                
\hline
1b                                                    & 2x2x                                          &          41.56                 &      0.9592                     &              43.31             &       0.9709 \\
1b                                                    & 4x                                          &          42.26                 &      0.9634                     &              44.45             &       0.9767

\\ \hline
\end{tabular}

% 1b                                                    & 2x2x                                          &          41.56                 &      0.9592                     &              43.31             &       0.9709 \\

==> srat/table/SR2.tex <==
\begin{tabular}{|c|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{2}{c|}{\textbf{SingleF}}                          & \multicolumn{2}{c|}{\textbf{SingleM}}                          \\ \cline{2-5} 
\multicolumn{1}{|c}{}                         & \multicolumn{1}{|c}{PSNR \uparrow} & \multicolumn{1}{|c}{SSIM $\uparrow$} & \multicolumn{1}{|c}{PSNR \uparrow} & \multicolumn{1}{|c|}{SSIM $\uparrow$} \\ \hline
Nearest                                        & 42.71                     & 0.9746                    & 44.68                     & 0.9821                    \\
Bilinear                                       & 44.38                     & 0.9797                    & 46.05                     & 0.9855                    \\
Bicubic                                        & 45.96                     & 0.9807                    & 47.39                     & 0.9885                    \\
DBPN~\cite{haris2018deep}                                           & 20.91                     & 0.3000                    & 19.73                     & 0.1188                    \\
SRFBN~\cite{li2019feedback}                                          & 17.12                     & 0.7583                    & 17.67                     & 0.7381                    \\
CSNLN~\cite{Mei_2020_CVPR}                                          & 48.12                     & 0.9900                    & 49.36                     & 0.9920                    \\
NLR~\cite{li20193d}                                            & 44.95                     & 0.9856                    & 46.73                     & 0.9888                    \\
NHR~\cite{li20193d}                                            & 34.81                     & 0.9788                    & 42.48                     & 0.9862                   \\
RCAN~\cite{zhang2018image}                                           & 48.14                     & 0.9900                    &        49.35                   &          0.9919                 \\
RCANtext               & 47.51                     & 0.9886                   &     48.50                      &             0.9904              \\ \
SRAT(ours)                    & \textbf{48.64}                     & \textbf{0.9912}                    & \textbf{50.45}                     & \textbf{0.9937}                    \\ 
\hline
\end{tabular}


==> srat/table/SR2new.tex <==
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Methods}}                  & \multicolumn{2}{c|}{\textbf{SingleF}}                                                & \multicolumn{2}{c|}{\textbf{SingleM}}                                                \\ \cline{2-5} 
                                                   & \multicolumn{1}{c|}{PSNR \uparrow} & SSIM $\uparrow$                  & \multicolumn{1}{c|}{PSNR \uparrow} & SSIM $\uparrow$                  \\ \hline
Bicubic                                            & 45.96                                             & 0.9807                           & 47.39                                             & 0.9885                           \\
DBPN~\cite{haris2018deep}    & 20.91                                             & 0.3000                           & 19.73                                             & 0.1188                           \\
SRFBN~\cite{li2019feedback}  & 17.12                                             & 0.7583                           & 17.67                                             & 0.7381                           \\
CSNLN~\cite{Mei_2020_CVPR} & 48.12                                             & 0.9900                           & 49.36                                             & 0.9920                           \\
NLR~\cite{li20193d}          & 44.95                                             & 0.9856                           & 46.73                                             & 0.9888                           \\
NHR~\cite{li20193d}          & 34.81                                             & 0.9788                           & 42.48                                             & 0.9862                           \\
RCAN~\cite{zhang2018image}   & 48.14                                             & 0.9900                           & 49.35                                             & 0.9919                           \\
RCANtext                                           & 47.51                                             & 0.9886                           & 48.50                                             & 0.9904                           \\
SRAT(ours)                         & \textbf{48.64}                   & \textbf{0.9912} & \textbf{50.45}                   & \textbf{0.9937} \\ \hline
CrossNet~\cite{zheng2018crossnet}                                          &     37.16                                              &                 0.9155                  & 38.96                                             & 0.9438                           \\
TTSR~\cite{yang2020learning}                                               & 41.29                                             & 0.9427                           & 43.00                                             & 0.9648                           \\
TTSR-\textit{$l_2$}               & 42.86                                             & 0.9622                           & 44.75                                             & 0.9759                           \\
SRNTT~\cite{zhang2019image}                                               & 42.92                                             & 0.9542                           & 43.86                                             & 0.9677                           \\
SRNTT-\textit{$l_2$}              & 44.11                                             & 0.9626                           & 45.26                                             & 0.9760                           \\ 
SRAT($4\times$)                         & \textbf{44.42}                   & \textbf{0.9636} & \textbf{45.57}                   & \textbf{0.9770} \\\hline
\end{tabular}

==> srat/table/SRnew.tex <==
\begin{tabular}{|ccc|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{Classic, GAN \& RefSR}}                                                                                 & \multicolumn{3}{c|}{\textbf{PSNR oriented}}                                                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{1}{c|}{\textit{\textbf{SingleI}}} & \textit{\textbf{SingleM}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{1}{c|}{\textbf{SingleI}} & \textbf{SingleM} \\ \cline{2-3} \cline{5-6} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{PSNR/SSIM}                 & PSNR/SSIM                 & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{PSNR/SSIM}        & PSNR/SSIM        \\ \hline
Bicubic                                                 &                                           &                         & SRResNet                                               & 44.00/.9621                           & 43.44/.9668      \\
Bilinear                                                &                 41.06/.9419                               &               42.16/.9630            & RRDBNet                                                & 44.12/.9626                           & 43.56/.9673      \\
Nearest                                                 &            39.08/.9157                                     &           39.99/.9424                & EDSR                                                   & 41.83/.9505                           & 43.31/.9664      \\
SRGAN                                                   & 37.31/.8850                                    & 39.17/.9272               & MDSR                                                   & 44.01/.9622                           & 43.37/.9664      \\
Cross-Net                                                  &                                    &             & CSNLN                                                  & 44.02/.9628                          &  45.17/.9761  \\
ESRGAN                                                  & 39.12/.9289                                    & 40.63/.9468               & RCAN                                                   & 44.09/.9625                           & 45.29/.9762     \\
RSRGAN                                                  & 42.36/.9528                                    & 42.97/.9651              & NHR                                                    & 30.35/.9441                                & 37.74/.9658           \\
SRNTT                                                   &                 43.16/.9553                   & 44.10/.9692      & NLR                                                    &       39.54/.9546                                &       42.74/.9703           \\
TTSR                                                    & 40.30/.9491                                    & 42.84/.9637               & SRNTTpsnr                                              &              44.13/.9626              &    45.29/.9762     \\
SRAT1                                                   & 43.38/.9571                                    & 44.20/.9701               & SRAT1psnr                                              &        44.09/.9623         &    45.23/.9759   \\
SRAT2                                                   & 43.41/.9573                                    &      44.24/.9707                    & SRAT2psnr                                              &                     44.16/.9627                  &   45.30/.9761   \\
SRAT4                                                   &            43.43/.9581                      &             44.40/.9716             & SRAT4psnr                                              &            44.17/.9627                           &          45.35/.9764        \\
SRAT8                                                   &                        43.40/.9576                        &          44.34/.9711                 & SRAT8psnr                   &           44.17/.9628                &            45.31/.9762                                            \\ \hline
\end{tabular}

==> srat/table/ablat.tex <==
\begin{tabular}{|ccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Config.}}} & \multicolumn{2}{c|}{\textbf{2 ref. images}}                                                     & \multicolumn{2}{c|}{\textbf{4 ref. images}}                                                     & \multicolumn{2}{c|}{\textbf{8 ref. images}}                                \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{\textit{\textbf{SingleF}}} & \multicolumn{1}{c|}{\textit{\textbf{SingleM}}} & \multicolumn{1}{c|}{\textit{\textbf{SingleF}}} & \multicolumn{1}{c|}{\textit{\textbf{SingleM}}} & \multicolumn{1}{c|}{\textit{\textbf{SingleF}}} & \textit{\textbf{SingleM}} \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{PSNR/SSIM}                                                                  & \multicolumn{2}{c|}{PSNR/SSIM}                                                                  & \multicolumn{2}{c|}{PSNR/SSIM}                                             \\ \hline
w $1^{st}$ module                                       & 43.41/.9581                                    & 44.24/.9707                                    & 43.43/.9573                                    & 44.40/.9716                                    &                                                &                           \\
w/o $1^{st}$ module                                     & 42.32/.9492                                    & 43.84/.9689                                    & 42.53/.9528                                    & 44.25/.9708                                    &                                                &                           \\ \hline
\end{tabular}

==> srat/table/pipes.tex <==

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Pipeline ID} & \textbf{Stage 1}                                                 & \textbf{Stage 2}                                                & \textbf{Stage 3}                                                          & \textbf{Stage 4}                                                          & \textbf{Stage 5}                                                          \\ \hline
1                    & \begin{tabular}[c]{@{}c@{}}Background\\ Elimination\end{tabular} & \begin{tabular}[c]{@{}c@{}}Couple\\ Identification\end{tabular} & \begin{tabular}[c]{@{}c@{}}Texture map\\ Retrieval\end{tabular}           & \begin{tabular}[c]{@{}c@{}}Colour transfer\\ of texture maps\end{tabular} & \begin{tabular}[c]{@{}c@{}}SR of texture\\ maps\end{tabular}              \\ \hline
2                    & \begin{tabular}[c]{@{}c@{}}Background\\ Elimination\end{tabular} & \begin{tabular}[c]{@{}c@{}}Couple\\ Identification\end{tabular} & \begin{tabular}[c]{@{}c@{}}Texture map\\ Retrieval\end{tabular}           & \begin{tabular}[c]{@{}c@{}}SR of texture\\ maps\end{tabular}              & \begin{tabular}[c]{@{}c@{}}Colour transfer\\ of texture maps\end{tabular} \\ \hline
3                    & \begin{tabular}[c]{@{}c@{}}Background\\ Elimination\end{tabular} & \begin{tabular}[c]{@{}c@{}}Couple\\ Identification\end{tabular} & \begin{tabular}[c]{@{}c@{}}Colour transfer\\ of input frames\end{tabular} & \begin{tabular}[c]{@{}c@{}}SR of corrected\\ frames\end{tabular}          & \begin{tabular}[c]{@{}c@{}}Texture map\\ Retrieval\end{tabular}           \\ \hline
4                    & \begin{tabular}[c]{@{}c@{}}Background\\ Elimination\end{tabular} & \begin{tabular}[c]{@{}c@{}}Couple\\ Identification\end{tabular} & \begin{tabular}[c]{@{}c@{}}SR of input\\ frames\end{tabular}              & \begin{tabular}[c]{@{}c@{}}Colour transfer\\ of input frames\end{tabular} & \begin{tabular}[c]{@{}c@{}}Texture map\\ Retrieval\end{tabular}           \\ \hline
5                    & \begin{tabular}[c]{@{}c@{}}Background\\ Elimination\end{tabular} & \begin{tabular}[c]{@{}c@{}}Couple\\ Identification\end{tabular} & \begin{tabular}[c]{@{}c@{}}SR of input\\ frames\end{tabular}              & \begin{tabular}[c]{@{}c@{}}Texture map\\ Retrieval\end{tabular}           & \begin{tabular}[c]{@{}c@{}}Colour transfer\\ of texture maps\end{tabular} \\ \hline
\end{tabular}

